M4GT-Bench: Evaluation Benchmark for Black-Box Machine-Generated Text Detection

The advent of Large Language Models (LLMs) has brought an unprecedented surge in machine-generated text (MGT) across diverse channels. This raises legitimate concerns about its potential misuse and societal implications. The need to identify and differentiate such content from genuine human-generated text is critical in combating disinformation, preserving the integrity of education and scientific fields, and maintaining trust in communication. In this work, we address this problem by introducing a new benchmark based on a multilingual, multi-domain, and multi-generator corpus of MGTs -- M4GT-Bench. The benchmark is compiled of three tasks: (1) mono-lingual and multi-lingual binary MGT detection; (2) multi-way detection where one need to identify, which particular model generated the text; and (3) mixed human-machine text detection, where a word boundary delimiting MGT from human-written content should be determined. On the developed benchmark, we have tested several MGT detection baselines and also conducted an evaluation of human performance. We see that obtaining good performance in MGT detection usually requires an access to the training data from the same domain and generators. The benchmark is available at https://github.com/mbzuai-nlp/M4GT-Bench.

==> section/multilingual_results.tex <==
\begin{table}[t!]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|l|cccc}
        \toprule
        Detector & Test & Prec & Recall & F1-score & Acc \\
        \midrule
        \multirow{7}{*}{XLM-R} & All & 91.49 & 98.52 & 94.86 & 94.52 \\
        &Indonesian & 53.13 & 100.0 & 69.39 & 55.83 \\
        &Chinese & 76.85 & 95.18 & 84.73 & 82.51 \\
        &Russian & 52.55 & 86.38 & 65.26 & 53.7 \\
        &Arabic & 88.91 & 97.35 & 92.64 & 92.18 \\
        &German & 66.21 & 98.3 & 79.0 & 73.62 \\
        &English & 63.72 & 84.64 & 72.42 & 66.51 \\

        \bottomrule
    \end{tabular}
}
    \caption{\textbf{Task 1 (multilingual): Binary human-written vs. machine-generated classification} performance on a test generator. Accuracy (Acc), Prec (precision), Recall, and F1-scores(\%) \textbf{with respect to machine-generated text}. The classifier was trained on the data of all languages except for the test language. \textit{All} refers to the setting that randomly splits train. validation and test sets, each has data of all languages.
    }
    \label{tab:subtaskA_multilingual}
\end{table}



==> section/outline.tex <==
What are major differences between previous work and what is our motivations?

Our major contributions:
1. We extend M4 datasets
2. We formulate new tasks for machine text detection
3. We do human evaluation over these new tasks and automatic baselines

Related work: How previous work frame machine-generated text detection, what’s new in our setting, why we frame in such a way. What’s the challenges in subtask C data collection?
Subtask definition: how we frame these tasks, it is our contributions, why this framing can be better to evaluate a detector’s performance.
Data collection: quality of the data. It is important to write descriptions to alleviate reviewer's concern about the data quality. We can only do it by manual checking since we do not have annotators. By sampling a subset, then human to check the quality. Then statistics.
Data analysis and human evaluation.
Experiments: models. Results and error analysis this time.
Conclusion and Future Work.
Highlight human evaluation, error analysis and future work, maybe some case studies for future work direction.


% temp table 7, without incorporating outfox data
\begin{table}[t!]
    \centering
     \small
    \tabcolsep2.5pt 
 %   \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|cccc}
        \toprule
        \multirow{2}{*}{\textbf{Detector}} & \textbf{Test} & \multicolumn{4}{c}{\textbf{Overall Performance}} \\ % & \multicolumn{7}{c}{Separate class F1-score} \\
        & \textbf{Domain} & \textbf{Prec} & \textbf{Recall} & \textbf{F1-macro} & \textbf{Acc}   \\%& Human & \davinci & \chatgpt & \gptfour & \cohere & \dolly & \bloomz \\
        \midrule
        \multirow{7}{*}{RoBERTa}
        & All & 96.35 & 96.21 & \textbf{96.23} & \textbf{96.25} \\ % & 96.34 & 94.43 & 96.38 & 96.74 & 97.12 & 93.30 & 99.31 \\
        & \arxiv & 60.55 & 41.11 & \underline{33.67} & \underline{41.11} \\ %& 44.91 & \textcolor{red}{0.49} & 27.97 & 64.61 & 2.28 & 38.91 & 56.49 \\
        & \peerread & 67.54 & 65.47 & 61.55 & 64.77 \\ % & 58.71 & \textcolor{red}{0.47} & 66.45 & 53.79 & 62.60 & 94.25 & 94.60 \\
        & \reddit & 73.59 & 67.97 & 62.33 & 67.97 \\ % & 89.89 & 10.38 & 50.14 & 29.12 & 84.72 & 77.12 & 94.92 \\
        & \wikihow & 70.94 & 67.60 & 64.91 & 64.20 \\ % & 27.95 & 39.25 & 50.45 & 86.94 & 67.46 & 83.72 & 98.57 \\
        & \wikipedia & 40.44 & 50.10 & 37.61 & 49.64 \\ % & 0.22 & \textcolor{red}{1.02} & 0.53 & 64.30 & 64.67 & 55.78 & 76.74 \\
        % & \outfox & 50.37 & 43.36 & 44.47 & 43.35\\
        \midrule
        \multirow{7}{*}{XLM-R}
        & All & 87.69 & 86.26 & \textbf{86.03} & \textbf{86.36} \\ % & 91.41 & 80.63 & 87.48 & 90.30 & 81.60 & 72.03 & 98.75 \\
        & \arxiv & 51.40 & 41.73 & 38.82 & 41.73  \\ %& 52.99 & 10.15 & 73.11 & 7.06 & 39.07 & 40.30 & 49.08 \\
        & \peerread & 52.20 & 51.66 & 44.84 & 50.38 \\ % & 17.19 & 0.53 & 66.21 & 32.68 & 38.51 & 62.64 & 96.13 \\
        & \reddit & 69.82 & 60.58 & 59.92 & 60.58 \\ % & 75.21 & 48.82 & 49.27 & 37.89 & 58.66 & 52.55 & 97.02 \\
        & \wikihow & 64.01 & 60.81 & 57.38 & 56.13 \\ % & 43.67 & 55.08 & 26.79 & 64.95 & 66.35 & 46.13 & 98.67 \\
        & \wikipedia & 58.57 & 41.07 & \underline{37.92} & \underline{40.25} \\ % & 8.42 & 40.51 & 31.51 & 36.79 & 38.28 & 48.21 & 61.70 \\
        % & \outfox & 33.22 & 29.62 & \underline{30.51} & \underline{29.62}\\
        \midrule
        \multirow{6}{*}{GLTR-LR}
        & All & 42.9 & 46.11 & 43.07 & 45.84 \\ % & 66.98 & 13.15 & 37.06 & 30.17 & 50.30 & 33.83 & 70.00 \\
        & \arxiv & 21.5 & 30.61 & \underline{23.19} & \underline{30.60} \\ % & 55.28 & 0.31 & 1.45 & 3.24 & 30.07 & 32.22 & 39.80 \\
        & \peerread & 43.50 & 46.24 & 42.52 & 46.37 \\ % & 58.77 & 1.05 & 36.18 & 50.92 & 43.31 & 39.51 & 67.90 \\
        & \reddit & 46.88 & 47.91 & \textbf{43.90} & \textbf{47.91} \\ % & 84.05 & 22.77 & 19.58 & 35.48 & 62.80 & 13.20 & 69.43 \\
        & \wikihow & 43.87 & 38.78 & 38.28 & 37.23 \\ % & 57.49 & 14.69 & 28.41 & 11.35 & 54.79 & 18.79 & 82.44 \\
        & \wikipedia & 41.91 & 35.66 & 35.54 & 34.08 \\ % & 67.54 & 11.78 & 14.10 & 20.12 & 32.22 & 33.90 & 69.14 \\
        \midrule
        \multirow{6}{*}{GLTR-SVM}
        & All & 53.19 & 53.47 & \textbf{52.50} & \textbf{53.75} \\ % & 70.15 & 32.16 & 53.37 & 42.57 & 53.57 & 41.41 & 74.28 \\
        & \arxiv & 27.88 & 35.40 & \underline{29.25} & \underline{35.40} \\ % & 61.14 & 0.06 & 42.95 & 0.00 & 28.55 & 33.7 & 38.33 \\
        & \peerread & 33.98 & 37.18 & 34.27 & 37.54 \\ % & 60.61 & 0.11 & 31.57 & 1.29 & 31.45 & 41.64 & 73.21 \\
        & \reddit & 46.68 & 47.84 & 44.73 & 47.84 \\ % & 83.34 & 14.95 & 43.89 & 18.88 & 56.88 & 15.58 & 79.62 \\
        & \wikihow & 43.88 & 42.36 & 40.52 & 37.84 \\ %& 66.13 & 22.54 & 1.15 & 23.16 & 64.09 & 23.65 & 82.93 \\
        & \wikipedia & 43.62 & 37.96 & 35.69 & 37.18\\ % & 53.55 & 17.18 & 40.28 & 43.48 & 32.03 & 36.89 & 26.45 \\
        \midrule
        \multirow{6}{*}{Stylistic-SVM}
        & All & 78.57 & 37.80 & \textbf{47.86} & \textbf{35.53} \\ %& 45.16 & 18.85 & 46.54 & 56.60 & 48.02 & 26.48 & 93.36 \\
        & \arxiv & 46.57 & 7.67 & \underline{11.55} & \underline{7.44} \\ %& 6.39 & 0.00 & 2.03 & 2.99 & 3.45 & 9.87 & 56.10 \\
        & \peerread & 53.40 & 27.16 & 30.39 & 25.30 \\ % &17.27 & 0.58 & 6.15 & 60.72 & 5.64 & 33.37 & 89.01 \\
        & \reddit & 61.96 & 28.23 & 33.07 & 26.53 \\ %& 50.18 & 15.22 & 10.78 & 26.11 & 29.06 & 12.92 & 87.18 \\
        & \wikihow & 54.48 & 34.89 & 39.94 & 26.49 \\ %& 43.20 & 26.8 & 29.77 & 38.6 & 25.26 & 23.34 & 92.60 \\
        & \wikipedia & 51.40 & 23.56 & 29.54 & 17.78 \\ % & 33.78 & 8.07 & 1.01 & 38.78 & 33.45 & 34.5 & 57.18 \\
        \midrule
        \multirow{6}{*}{NELA-SVM}
        & All & 66.99 & 27.48 & \textbf{34.80} & \textbf{25.60} \\ %& 37.64 & 0.36 & 18.63 & 30.52 & 48.00 & 14.75 & 93.72 \\
        & \arxiv & 53.46 & 12.97 & \underline{19.11} & \underline{11.71} \\ %& 13.64 & 0.07 & 12.88 & 10.73 & 19.00 & 10.81 & 66.62 \\
        & \peerread & 48.53 & 24.76 & 22.84 & 23.31 \\ %& 7.80 & 0.00 & 5.1 & 41.17 & 9.59 & 4.72 & 91.50 \\
        & \reddit & 45.94 & 28.09 & 31.45 & 24.20 \\ % & 49.00 & 0.46 & 8.69 & 8.32 & 48.28 & 13.96 & 91.43 \\
        & \wikihow & 46.87 & 24.81 & 28.54 & 21.16 \\ % & 48.68 & 0.20 & 6.96 & 13.88 & 16.80 & 16.65 & 96.59 \\
        & \wikipedia & 47.81 & 22.62 & 27.36 & 19.79 \\ % & 31.19 & 0.07 & 6.88 & 5.79 & 29.46 & 24.95 & 93.19 \\
        \bottomrule
    \end{tabular}
%    }
    \caption{\textbf{Task 2: multi-generator detection accuracy without incorporating \outfox.} Classifiers are trained on the data of all domains except for the test domain (unseen). \textit{All} refers to the setting that randomly split train, validation and test sets, each has data of all domains. Given a detector, bold is the best and the underlined is the worst Acc and F1-macro.}
    \label{tab:subtaskB}
\end{table}
